SL-CBM: Enhancing Concept Bottleneck Models with Semantic Locality for Better Interpretability

Explainable AI (XAI) is crucial for building transparent and trustworthy machine learning systems, especially in high-stakes domains. Concept Bottleneck Models (CBMs) have emerged as a promising ante-hoc approach that provides interpretable, concept-level explanations by explicitly modeling human-understandable concepts. However, existing CBMs often suffer from poor locality faithfulness, failing to spatially align concepts with meaningful image regions, which limits their interpretability and reliability. In this work, we propose SL-CBM (CBM with Semantic Locality), a novel extension that enforces locality faithfulness by generating spatially coherent saliency maps at both concept and class levels. SL-CBM integrates a 1x1 convolutional layer with a cross-attention mechanism to enhance alignment between concepts, image regions, and final predictions. Unlike prior methods, SL-CBM produces faithful saliency maps inherently tied to the model's internal reasoning, facilitating more effective debugging and intervention. Extensive experiments on image datasets demonstrate that SL-CBM substantially improves locality faithfulness, explanation quality, and intervention efficacy while maintaining competitive classification accuracy. Our ablation studies highlight the importance of contrastive and entropy-based regularization for balancing accuracy, sparsity, and faithfulness. Overall, SL-CBM bridges the gap between concept-based reasoning and spatial explainability, setting a new standard for interpretable and trustworthy concept-based models.

==> tex/checklist.tex <==
\section*{Reproducibility Checklist}

\newcommand{\yes}[0]{{\color{blue}{\textbf{Yes}}}}
\newcommand{\no}[0]{{\color{blue}{\textbf{No}}}}
\newcommand{\na}[0]{{\color{blue}{\textbf{NA}}}}
\newcommand{\PaRtial}[0]{{\color{blue}{\textbf{Partical}}}}


\subsection{General Paper Reproducibility}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) \yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) \yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) \yes
\end{itemize}

\subsection{Theoretical Contributions}

Does this paper make theoretical contributions? (yes/no) \yes

If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) \yes
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) \yes
    \item Proofs of all novel claims are included. (yes/partial/no) \no
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) \yes
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no) \yes
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) \yes
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) \yes
\end{itemize}


\subsection{Dataset Usage}

Does this paper rely on one or more datasets? (yes/no) \yes

If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) \yes
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) \na
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) \na
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) \yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) \yes
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \na
\end{itemize}

\subsection{Computational Experiments}

Does this paper include computational experiments? (yes/no) \yes

If yes, please complete the list below.

\begin{itemize}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) \yes
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).  \yes
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) \yes
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \yes
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \yes
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \yes
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \yes
    \item  This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \yes
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \yes
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) \yes
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) \no
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) \yes
\end{itemize}


























==> tex/old.tex <==
abstract
\begin{itemize}
    \item Briefly summarize the study’s goal: exploring how concept bottleneck models can bridge adversarial examples and counterfactual explanations in visual tasks.
    \item improved explainability with respect to saliency maps and counterfactual explanations after adversarial fine-tuning.
    \item proposing a novel adversarial fine-tuning approach on CLIP models using concept bottleneck networks for enhanced explainability.
\end{itemize}

introduction
\begin{itemize}
    \item Briefly introduce adversarial examples, counterfactual explanations, and their roles in explainable AI.
    \item Highlight the similarity in problem formulation but the difference in desired properties between adversarial examples (non-semantic perturbations) and counterfactual explanations (semantically meaningful changes).
    \item Why understanding and improving the relationship between these concepts in visual tasks is important.
    \item Mention the limitations of current concept bottleneck models in providing reliable explanations, as shown by saliency map evaluations.
    \item To develop a method using adversarial fine-tuning on concept bottleneck-enhanced CLIP models, aiming to improve explainability.
    \item contribution: 
    \begin{itemize}
        \item Analyze the connection between adversarial examples and counterfactual explanations using concept bottlenecks.
        \item Design and evaluate adversarial fine-tuning on CLIP with post-hoc concept bottleneck models.
        \item Experiment on different model backbones (CNN and transformer) and benchmark datasets.
    \end{itemize}
\end{itemize}

related work
\paragraph{Concept Bottleneck Models (CBM)}

Current CBM variants suffer from a trade-off between model performance and interpretabilty\cite{espinosa2022concept} 


TCAV~\cite{kim2018interpretability}
CBM~\cite{koh2020concept}
probabilityCBM~\cite{kim2023probabilistic}
visual-TCAV~\cite{de2024visual}

concept explanation, concept saliency map
improving the accuracy of class/concept, improving the alignment between class and concept, improving the concept saliency map, improving the explanation of cbm

\paragraph{Explainability in Neural Networks}

method

\subsection{Problem Formulation}

\paragraph{Adversarial Examples}
\paragraph{Counterfactual Explanation}

\paragraph{CBM as a Bridge}

\subsection{Proposed Approach: Adversarial Fine-tuning}

\begin{itemize}
    \item Adversarial Loss
    \item Architecture
    \item Fine-tuning scheme
\end{itemize}

experiments


\paragraph{Model}
Clip Backbone: (1) Transformer-based; (2) CNN-based
CBM: PHCBM

\paragraph{Dataset}
Cifar 10/100
CUB
ImageNet

\paragraph{Evaluation Metrics}
(1) Saliency map coherence (evaluating adversarial and counterfactual alignment)
(2) Counterfactual explanation quality (semantic relevance of generated examples)

\paragraph{Saliency Map Method}

\emph{Integrated Gradient (IG)}
\emph{GradCAM}


\subsection{Concept Bottleneck Analysis}


Compare results before and after adversarial fine-tuning to assess the impact on explainability.

\begin{itemize}
    \item Train concept bottleneck models with both CNN and transformer (e.g., CLIP) backbones on chosen datasets.
    \item Generate adversarial examples for each model, ensuring they focus on non-semantic perturbations.
    \item Use CBMs to interpret adversarial examples in terms of relevant concepts.
    \item Conduct a preliminary evaluation of the saliency maps to establish a baseline for explainability before fine-tuning.
\end{itemize}

\paragraph{Does CBM learn the correct saliency of concept?}

We feed an image to the PHCBM, then we choose the top 5 concepts by
\begin{itemize}
    \item (1) score of the concepts;
    \item (2) weight of the concepts contributing to the predicted class.
\end{itemize}
First, we should know the overlap of (1) and (2).
Second, we generate saliency maps using IG and GradCAM based on the top 5 concepts identified from (1) and (2).

We can randomly select a subset of images for the experiment and display the visualizations of the saliency maps generated by the two methods.

% \input{tex/table/visual_saliency}

\paragraph{What is the original adversarial robustness of the PHCBM?}
We only consider the successfully predicted examples and apply attacks on these examples. We use PGD as the attack method, and test a set of $\epsilon \in [0.01,0.05,0.1,0.3,0.5]$ (please check what is reasonable number, and we only need to test three value of $\epsilon$)
\begin{itemize}
    \item[A] we attack the groundtruth class (standard untargeted attack loss), and we report the ASR in this case, and compare the score of concept before and after attacking.
    \item[B] We select the top 5 concepts, and reduce the score of the concepts, then we report the score of the concepts after attacking, and ASR of groundtruth class.
\end{itemize}

Homework: 

\begin{table*}[]
    \centering
    \begin{tabular}{ll|ccc}
     backbone & loss& class accuracy   & concept accuracy &  IoU  \\
         PCBM+RN50 & cross entropy loss & 91.0 &	48.63 &	0.0944 \\
         PCBM+ViTB16 & cross entropy loss & 90.01 &	40.07 &	0.0895  \\
         CSS-VLM & contractive loss + cross entropy loss + L1 concept loss & 97.94 &	87.69 &	0.0997  \\
    \end{tabular}
    \caption{Test different methods}
    \label{tab:my_label}
\end{table*}


\begin{table*}[]
    \centering
    \begin{tabular}{lll|ccccc}
       class cross-entropy loss& concept l1 loss& entropy loss& class accuracy   & concept accuracy &  IoU &  Dice &  Precision IoU  \\
        1.0 & 1e4 & 0.0 & 99.26 & 90.26 &	0.1356 & 0.1921 & 0.2917 \\
        1.0 & 1e4 & 0.1 & 99.26	& 90.11 &	0.1218 & 0.1756 & 0.2543 \\
        1.0 & 1e4 & 0.5 & 99.38 & 90.05 &	0.1246 & 0.1756 & 0.2703 \\
        1.0 & 1e4 & 1.0 & 99.28 & 89.83 &	0.1177 & 0.1697 & 0.2616 \\
        1.0 & 1e4 & 1.5 & 99.39 & 89.12 &	0.1214 & 0.1784 & 0.3024 \\
    \end{tabular}
    \caption{Using our structure, ablation with different weight of loss}
    \label{tab:my_label}
\end{table*}

\begin{table*}[]
    \centering
    \begin{tabular}{lll|ccccc}
       class cross-entropy loss& concept l1 loss& entropy loss& class accuracy   & concept accuracy &  IoU &  Dice &  Precision IoU  \\
        1.0 & 1e4 & 0.0 & 99.19 & 90.09 &	0.0984 & 0.1486 & 0.1719 \\
        1.0 & 1e4 & 0.1 & 99.19	& 90.15 &	0.0917 & 0.1385 & 0.1684 \\
        1.0 & 1e4 & 0.5 & 99.17 & 89.98 &	0.0788 & 0.1193 & 0.1605 \\
        1.0 & 1e4 & 1.0 & 99.17 & 89.64 &	0.0772 & 0.1159 & 0.1640 \\
        1.0 & 1e4 & 1.5 & 98.54 & 88.98 &	0.0923 & 0.1482 & 0.4341 \\
    \end{tabular}
    \caption{Using our structure with softmax, ablation with different weight of loss}

\end{table*}

\subsection{Adversarial Fine-Tuning}
Fine-tune both CNN and transformer-based models using adversarial examples filtered through the concept bottleneck model. 

Adjust hyperparameters to optimize the fine-tuning process, aiming to preserve semantic interpretability while improving robustness.

\paragraph{Loss}

Baseline: ASGT (cross-entropy + adv training + KL)

1. cross-entropy ($\checkmark$)


2 adv training cross-entropy  ($\checkmark$)
3 adv v.s ori (embedding) 


4 saliency masked v.s. ori (KL in class logit; concept score)

5 regularization on saliency mask (L0; L1 norm, saliency map should not take all the image)

6 concept competition (several concept saliency maps summing up to 1 for each pixel)

7 contrastive learning of concepts (maximize the distance between classes and concepts)


Step 1: Modification on KL, check 4-7  

\paragraph{Fine-tuning setting}
- image encoder
- PH CBM
- text encoder (optional, CUB doesn't have it)

\paragraph{Evaluate Concept Explanability}

- Localization: concept segmentation notation (SAM)





\paragraph{Quantitative Results}
\begin{itemize}
    \item Compare the quality of saliency maps and counterfactual explanations for CNN-based and transformer-based backbones.
    \item Statistical analysis of improvements in explanation quality after adversarial fine-tuning.
\end{itemize}
\paragraph{Qualitative Analysis}
\begin{itemize}
    \item Visualization of saliency maps and counterfactual examples to demonstrate the increased semantic relevance after fine-tuning.
    \item Case studies illustrating the interpretability of adversarially fine-tuned models compared to baseline.
\end{itemize}


% \begin{table*}[]
%     \centering
%     \begin{tabular}{llll|ccccc}
%        class & concept&  E & C & class accuracy   & concept accuracy &  IoU &  Dice &  Precision IoU  \\
%         1.0 & 1e4 & 0.0 & 0.0 & 98.81 &	89.82 &	0.34 &	0.41 &	0.34 \\
%         1.0 & 1e4 & 0.1 & 0.0 & 99.19 &	89.92 &	0.37 &	0.43 &	0.37 \\
%         1.0 & 1e4 & 0.5 & 0.0 & 98.98 &	89.93 &	0.32 &	0.37 &	0.32 \\
%         1.0 & 1e4 & 1.0 & 0.0 & 99.15 &	89.85 &	0.41 &	0.46 &	0.41 \\
%         1.0 & 1e4 & 1.5 & 0.0 & 99.32 &	89.94 &	0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 2.0 & 0.0 & 99.30 &	89.92 &	0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 5.0 & 0.0 & 99.30 &	90.07 &	0.44 &	0.49 &	0.44 \\
%         1.0 & 1e4 & 10.0 & 0.0 & 99.11 & 85.86 & 0.43 &	0.47 &	0.43 \\
        
%         \hline 
%         1.0 & 1e4 & 0.0 & 1.0 & 99.32 &	90.34 &	0.37 &	0.43 &	0.37 \\
%         1.0 & 1e4 & 0.1 & 1.0 & 99.24 &	90.17 &	0.36 &	0.42 &	0.36 \\
%         1.0 & 1e4 & 0.5 & 1.0 & 99.11 &	90.23 &	0.35 &	0.41 &	0.35 \\
%         1.0 & 1e4 & 1.0 & 1.0 & 99.11 &	90.01 & 0.41 &	0.46 &	0.41 \\
%         1.0 & 1e4 & 1.5 & 1.0 & 99.38 &	90.13 &	0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 2.0 & 1.0 & 99.19 &	89.92 &	0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 5.0 & 1.0 & 99.13 &	89.93 &	0.45 &	0.50 &	0.45 \\
%         1.0 & 1e4 & 10.0 & 1.0 &99.28 &	86.54 &	0.44 &	0.48 &	0.44 \\
%     \end{tabular}
%     \caption{Using our structure, ablation with different weight of loss}
%     \label{tab:my_label}
% \end{table*}



% \begin{table*}[]
%     \centering
%     \begin{tabular}{llll|ccccc}
%        class & concept&  E & C & class accuracy   & concept accuracy &  IoU &  Dice &  Precision IoU  \\
%         1.0 & 1e4 & 0.0 & 0.0 &  98.85 & 89.69 & 0.34 &	0.40 &	0.34 \\
%         1.0 & 1e4 & 0.1 & 0.0 & 99.05 &	89.53 &	0.44 &	0.49 &	0.44 \\
%         1.0 & 1e4 & 0.5 & 0.0 & 98.79 &	89.59 &	0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 1.0 & 0.0 & 98.68 &	89.62 &	0.42 &	0.46 &	0.42 \\
%         1.0 & 1e4 & 1.5 & 0.0 & 98.79 &	89.26 &	0.42 &	0.46 &	0.42 \\

%         1.0 & 1e4 & 2.0 & 0.0 & 98.6 &	89.02 & 0.42 &	0.47 &	0.42 \\
%         1.0 & 1e4 & 5.0 & 0.0 & 94.55 &	82.35 &	0.41 &	0.45 &	0.41 \\
%         1.0 & 1e4 & 10.0 & 0.0 & 65.29 & 64.31 & 0.42 &	0.44 &	0.42 \\
%         \hline
%         1.0 & 1e4 & 0.0 & 1.0 & 98.94 &	89.65 &	0.34 &	0.40 &	0.34 \\
%         1.0 & 1e4 & 0.1 & 1.0 & 99.02 &	89.53 &	0.44 &	0.49 &	0.44 \\
%         1.0 & 1e4 & 0.5 & 1.0 & 98.5 &	89.39&	0.45 &	0.50 &	0.45 \\
%         1.0 & 1e4 & 1.0 & 1.0 & 98.39 &	89.02 & 0.41 &	0.45 &	0.41 \\
%         1.0 & 1e4 & 1.5 & 1.0 & 98.58 &	88.80 &	0.42 &	0.46 &	0.42 \\

%         1.0 & 1e4 & 2.0 & 1.0 & 98.50 &	89.15 &	0.43 &	0.47 &	0.43 \\
%         1.0 & 1e4 & 5.0 & 1.0 & 97.77 &	82.06 &	0.43 &	0.47 &	0.43 \\
%         1.0 & 1e4 & 10.0 & 1.0 & 57.86 & 62.18 & 0.40 &	0.43 &	0.40 \\

%     \end{tabular}
%     \caption{Using our structure with softmax, ablation with different weight of loss}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{ll|ccccc} \toprule
%      backbone & loss& class accuracy   & concept accuracy &  IoU & Dice & C-IoU  \\
%          RN50 & cross entropy loss & 91.0 &	48.63 &	0.21 &	0.24 &	0.21 \\
%          ViTB16 & cross entropy loss & 90.01 &	40.07 & 0.14 &	0.17 & 0.14 \\
%          CSS & css-vlm loss & 97.94 &	87.69 &	0.38 & 0.44 & 0.38\\ 
         
%          \bottomrule
%     \end{tabular}
%     \caption{Test different methods}
%     \label{tab:my_label}
% \end{table*}
% \end{table*}

% We use the RIVAL-10 dataset~\cite{moayeri2022comprehensive}\footnote{The dataset is sourced from \url{https://mmoayeri.github.io/RIVAL10/index.html}.}, which maps CIFAR-10~\cite{krizhevsky2009learning} classes to ImageNet~\cite{krizhevsky2012imagenet} and comprises approximately 26,000 images. Each image includes 18 visual attributes, as well as attribute and object segmentations. We train on 21,098 images and test on 5,286, reporting all results on the test set.
% Additionally, we use the CUB-200-2011 dataset~\cite{WahCUB_200_2011}\footnote{The dataset is sourced from \url{https://www.vision.caltech.edu/datasets/cub_200_2011/}}, a benchmark for fine-grained visual categorization, containing 11,788 images across 200 bird subcategories. It provides detailed annotations, including part locations, attributes, and bounding boxes. We use 4,796 images for training and 5,794 for testing, reporting results on the test set. When using CUB, we adopt the setup of PCBM~\cite{yuksekgonul2022post} by employing an imbalanced dataset sampler.

% We select two state-of-the-art CBMs for comparison, \ie PCBM~\cite{yuksekgonul2022post}\footnote{The codes are sourced from: \url{https://github.com/mertyg/post-hoc-cbm}} and CCS~\cite{singhi2024improving}\footnote{The codes are sourced from: \url{https://github.com/NMS05/Improving-Concept-Alignment-in-Vision-Language-Concept-Bottleneck-Models}}. We evaluate two versions of PCBM, using ResNet50 and ViT-B16 as the backbone. CSS uses a ViT-B16-based CLIP model as the backbone and is trained with the same parameters as in the original version.
% Our SL-CBM employs a ViT-B16-based CLIP model\footnote{The pre-trained weights are sourced from: \url{https://huggingface.co/laion/CLIP-ViT-B-16-laion2B-s34B-b88K}} as the backbone. We train SL-CBM with a learning rate of $0.0003$ using the Adam optimizer. By default, the loss function is combined with $\lambda_{ce}=1$, $\lambda_{ca}=10^4$, $\lambda_e=5$, and $\lambda_c=0$.
% We choose ResNet~\cite{he2016deep} as a representation of computer vision backbone, we use ResNet18\footnote{The pre-trained weights are sourced from PyTorch.} for testing the adaptability of the CBMs. We set $\lambda_e=1.0$ for SL-CBM in this setting while keeping the remaining parameters unchanged.

% We visualize the saliency maps at both the concept and class levels in \autoref{fig:top5-concept-class}, showing the top five concepts for each CBM. When comparing the CNN-based backbone to the transformer-based backbone in PCBM, we observe that the CNN-based backbone is more compact.
% PCBM, based on ViT-B16, shares the same backbone as CSS and SL-CBM. We observe that GradCAM produces unreliable saliency maps for both PCBM and CSS, failing to capture proper localization but ends up with correct prediction. In contrast, SL-CBM achieves better localization along with prediction. For example, the saliency map for the concept \emph{Break} in SL-CBM includes only relevant regions and avoids covering the entire image, unlike other CBMs with different transformer backbones. Additionally, SL-CBM learns distinct saliency maps for different concepts, improving its localization capabilities. Since SL-CBM generates saliency maps inherently, we can conclude that it fails to learn the concept \emph{Tail} for the given image. However, for other methods, this cannot be determined as their reliance on GradCAM makes it unclear whether the issue lies with GradCAM itself or the CBMs.
% This case highlights a limitation of SL-CBM: while it improves locality faithfulness, its performance in providing explanations heavily depends on the quality of the concepts. SL-CBM does not include a strategy to improve concept quality, but it can be easily combined with existing methods to further enhance performance.


% In this work, we introduce the concept of SL-CBM (CBM with Semantic Locality) to address the limitations of traditional CBMs in terms of locality faithfulness and class-concept alignment. By incorporating both concept-level and class-level saliency maps, SL-CBM enhances the explainability of model predictions while ensuring that the saliency maps are faithful to the underlying concepts and their locality. Through the use of techniques, such as cross-attention and a $1 \times 1$ convolutional layer for saliency map generation, we demonstrate that SL-CBM provides a more interpretable and accurate method for understanding model behavior. Our approach not only improves concept and class accuracy but also ensures sparsity and simplicity in the generated saliency maps, which are crucial for high-quality explainable AI. The experimental results validate the effectiveness of SL-CBM in achieving locality faithfulness and providing more insightful explanations compared to traditional saliency methods. Ultimately, our work contributes to the advancement of explainable AI, offering a promising framework for building more transparent and trustworthy models in real-world applications.

==> tex/table/table-CUB-planB.tex <==
\begin{table}[]
    \centering
    \setlength{\tabcolsep}{5.5pt}
    \begin{tabular}{l|cc|ccc} \toprule
     {\mr{2}{Method}}  & \multicolumn{2}{c|}{{Accuracy}} & \mc{3}{Locality Faithfulness} \\\cmidrule{2-6}
     &  Concept & Class & {AD $\downarrow$}& {AI $\uparrow$}& {AG $\uparrow$}\\\midrule
     PCBM      & \textbf{69.37} & 60.03 & 7.94& 28.52& 2.51\\\midrule
        CSS  & 58.4 &\textbf{ 51.43} & \textbf{2.32}&  36.14&1.44\\ \midrule
         \rowcolor{cyan!10}
     SL-CBM  & 69.33 & \textbf{84.93} & 5.32& \textbf{49.52}&  \textbf{12.28}\\
         \bottomrule
    \end{tabular}
    \caption{Comparison of SL-CBM with state-of-the-art CBMs on CUB in terms of both concept-level and class-level accuracy, as well as locality faithfulness metrics without annotation (AD, AI, AG) at concept-level. $\uparrow$ signifies that a higher value is preferable for the metric, while $\downarrow$ indicates that a lower value is better. All values are presented as percentages. The best results are highlighted in bold.}
    \label{tab:cp-CUB}
\end{table}

==> tex/table/table_celebA.tex <==

\begin{table*}[thbp]
    \centering
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{lr|cc|cc|cc|cc|cc} \toprule
     \multicolumn{2}{c|}{\mr{4}{Method}} & \multicolumn{4}{c|}{\mr{3}{Accuracy}} & \mc{6}{Locality Faithfulness (Without Annotation)} \\\cmidrule{7-12}
     &&\multicolumn{4}{c|}{} &\multicolumn{2}{c|}{AD $\downarrow$}&\multicolumn{2}{c|}{AI $\uparrow$}&\multicolumn{2}{c}{AG $\uparrow$}\\ \cmidrule{3-12}
     && Concept&Class & NEC-5& ANEC &$S_{\cC_{gt}}$&$S_{l_{gt}}$&$S_{\cC_{gt}}$&$S_{l_{gt}}$&$S_{\cC_{gt}}$&$S_{l_{gt}}$\\\midrule
         \mr{2}{PCBM}&ResNet50 & 47.52 & 72.46 & 72.46 & 72.46 & 1.06 & 1.15 & 29.86 & 25.54 & 0.36 & 0.28 \\
         &ViT-B16 &  42.36 & 67.53 & 60.71 & 64.12 & \textbf{0.37} & \textbf{0.37} & \textbf{83.34} & \textbf{82.68} & \textbf{25.63} & \textbf{22.96}\\\midrule
        \multicolumn{2}{c|}{CSS} & 71.54 & \textbf{91.27} & \textbf{91.21} & \textbf{91.24} & 24.16 & 26.42 & 45.63 & 41.46 & 21.80 & 19.88\\ \midrule
         \rowcolor{cyan!10}
          \multicolumn{2}{c|}{SL-CBM}& \textbf{77.37} & 85.99 & 85.82 & 85.91 & 23.11 & 21.32 & 42.21 & 42.19 & 17.14 & 14.69\\
         \bottomrule
    \end{tabular}
    \caption{Comparison of SL-CBM with state-of-the-art CBMs on CelebA in terms of accuracy, as well as locality faithfulness metrics with annotation (IoU, Dice, C-IoU) and without annotation (AD, AI, AG) at both concept-level and class-level. $\uparrow$ signifies that a higher value is preferable for the metric, while $\downarrow$ indicates that a lower value is better. All values are presented as percentages. The best results are highlighted in bold.}
    \label{tab:cp-celeba}
\end{table*}

==> tex/table/table_trans.tex <==
\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lr|cc|cc|cc|cc|cc} \toprule
     \multicolumn{2}{c|}{\mr{4}{Method}} & \multicolumn{4}{c|}{\mr{3}{Accuracy}} & \mc{6}{Locality Faithfulness (Without Annotation)} \\\cmidrule{7-12}
     &&\multicolumn{4}{c|}{} &\multicolumn{2}{c|}{AD $\downarrow$}&\multicolumn{2}{c|}{AI $\uparrow$}&\multicolumn{2}{c}{AG $\uparrow$}\\ \cmidrule{3-12}
     && Concept&Class & NEC-5& ANEC &$S_{\cC_{gt}}$&$S_{l_{gt}}$&$S_{\cC_{gt}}$&$S_{l_{gt}}$&$S_{\cC_{gt}}$&$S_{l_{gt}}$\\\midrule
         \mr{2}{PCBM}&ResNet50 & 76.19 &	54.52 & 54.52 & 54.52 & 0.43 & 0.44 & 60.64 & 60.23 & \textbf{1.03} & \textbf{1.04} \\
         &ViT-B16 &  77.81 &	56.36 & 56.36 & 56.36 & \textbf{0.36} &\textbf{0.36}& \textbf{75.09}& \textbf{74.77} & 17.62 & 17.37\\\midrule
        \multicolumn{2}{c|}{CSS} & 81.87 & \textbf{90.28} & \textbf{90.28} & \textbf{90.28} & 3.09 & 2.76 & 47.27 & 46.27 & 1.30 & 1.24\\ \midrule
         \rowcolor{cyan!10}
          \multicolumn{2}{c|}{SL-CBM}& \textbf{82.83} & 89.19 & 88.39& 88.93 & 22.64 & 21.37 & 49.37 &  49.60 & 12.09 & 11.57\\
         \bottomrule
    \end{tabular}
    \caption{Transferability of RIVAL10.}
    \label{tab:cp-trans}
\end{table*}

